Diagnosing Model Performance Under Distribution Shift

Prediction models can perform poorly when deployed to target distributions different from the training distribution. To understand these operational failure modes, we develop a method, called DIstribution Shift DEcomposition (DISDE), to attribute a drop in performance to different types of distribution shifts. Our approach decomposes the performance drop into terms for 1) an increase in harder but frequently seen examples from training, 2) changes in the relationship between features and outcomes, and 3) poor performance on examples infrequent or unseen during training. These terms are defined by fixing a distribution on $X$ while varying the conditional distribution of $Y \mid X$ between training and target, or by fixing the conditional distribution of $Y \mid X$ while varying the distribution on $X$. In order to do this, we define a hypothetical distribution on $X$ consisting of values common in both training and target, over which it is easy to compare $Y \mid X$ and thus predictive performance. We estimate performance on this hypothetical distribution via reweighting methods. Empirically, we show how our method can 1) inform potential modeling improvements across distribution shifts for employment prediction on tabular census data, and 2) help to explain why certain domain adaptation methods fail to improve model performance for satellite image classification.

==> tables/adult_x_kids_4.tex <==

        \begin{tabular}{lcccc}
            \toprule
            & & \multicolumn{3}{c}{Standard error} \\
            \cmidrule(lr){3-5}
            Term & Estimate & NP boot & HS boot & IF est \\
            \midrule
 $\E_P[R_P(\feature)]$ & 83.50\%  & 0.38\%  & 0.37\%  & 0.38\% \\
 $\E_{{S_Z}}[R_P(\feature)]$ & 83.27\%  & 0.40\%  & 0.49\%  & 0.54\% \\
 $\E_{{S_Z}}[R_Q(\feature)]$ & 83.28\%  & 0.36\%  & 0.37\%  & 0.40\% \\
 $\E_Q[R_Q(\feature)]$ & 66.08\%  & 0.25\%  & 0.27\%  & 0.00\% \\        
            \bottomrule
        \end{tabular}
    

==> tables/adult_x_oversample_4.tex <==

        \begin{tabular}{lcccc}
            \toprule
            & & \multicolumn{3}{c}{Standard error} \\
            \cmidrule(lr){3-5}
            Term & Estimate & NP boot & HS boot & IF est \\
            \midrule
 $\E_P[R_P(\feature)]$ & 76.95\%  & 0.80\%  & 0.76\%  & 0.76\% \\
 $\E_{{S_Z}}[R_P(\feature)]$ & 74.92\%  & 0.86\%  & 0.94\%  & 1.23\% \\
 $\E_{{S_Z}}[R_Q(\feature)]$ & 74.64\%  & 0.66\%  & 0.73\%  & 0.89\% \\
 $\E_Q[R_Q(\feature)]$ & 69.49\%  & 0.53\%  & 0.51\%  & 0.01\% \\        
            \bottomrule
        \end{tabular}
    

==> tables/adult_yx_4.tex <==

        \begin{tabular}{lcccc}
            \toprule
            & & \multicolumn{3}{c}{Standard error} \\
            \cmidrule(lr){3-5}
            Term & Estimate & NP boot & HS boot & IF est \\
            \midrule
 $\E_P[R_P(\feature)]$ & 69.68\%  & 0.79\%  & 0.77\%  & 0.76\% \\
 $\E_{{S_Z}}[R_P(\feature)]$ & 68.90\%  & 0.84\%  & 0.98\%  & 1.05\% \\
 $\E_{{S_Z}}[R_Q(\feature)]$ & 62.61\%  & 0.80\%  & 0.91\%  & 0.92\% \\
 $\E_Q[R_Q(\feature)]$ & 61.26\%  & 0.61\%  & 0.64\%  & 0.01\% \\        
            \bottomrule
        \end{tabular}
    

==> wilds.tex <==
\subsection{DANN model on WILDS-FMOW}
We also demonstrate our method on 
natural distribution shifts on predicting land use from satellite imagery
in different regions and years
in the WILDS-FMOW dataset in~\cite{KohSaEtAl20,SagawaKoLeGaXiShKuHuYaMa21}.
In particular, worst-region model performance degrades substantially
between training and test datasets\footnote{
The training set consists of data before 2013, while the test set
consists of data from 2016 and after.
The validation set consists of the years in between.}, \tc{check leaderboard?}
even for a variety of models that use domain-adaptation methods. 
It is currently not well-understood why model performance degrades so much
between training and test distributions. 



We focus on domain-adversarial neural networks (DANN)
\cite{GaninUsAjGeLaLaMaLe16},
which try to learn feature representations that 
are similar between domains by penalizing representations 
for which an auxiliary classifier can discriminate between
domains. 
From the point of view of our framework, DANN models try to learn
features $X$ \tc{ugh, notation} for which $P_X$ is similar to $Q_X$.
DANN assumes that $Y|X$ is the same between domains. 
Thus, we wonder how much of the performance degradation
our method will attribute to $X$ vs $Y|X$ shifts. 
If there is substantial $X$ shift, this would suggest that
the DANN method did not result in features that are indistinguishable
between domains. If there is substantial $Y|X$ shift, 
this would suggest that the assumption that $Y|X$ is the same between domains
does not hold. 

\tc{todo}

\tc{interventions???}
Observe that in the pursuit of good performance on deployment distributions,
our diagnostic is not obviated by methods that are designed to perform well across
shifts; rather, our diagnostic complements them.


